Interpretation of the Depths of Maximum of Extensive Air Showers Measured by the Pierre Auger Observatory

To interpret the mean depth of cosmic ray air shower maximum and its dispersion, we parametrize those two observables as functions of the first two moments of the $\ln A$ distribution. We examine the goodness of this simple method through simulations of test mass distributions. The application of the parameterization to Pierre Auger Observatory data allows one to study the energy dependence of the mean $\ln A$ and of its variance under the assumption of selected hadronic interaction models. We discuss possible implications of these dependences in term of interaction models and astrophysical cosmic ray sources.

==> compile <==
#!/usr/bin/perl
# Author F. Salamida

use strict;
use warnings;

my $argc = @ARGV;
###print "$argc\n";
if ($argc<1) {
    print "USAGE: ./compile filename.tex\n";
    exit;
}

my $file = $ARGV[0];


for (my $count = 0; $count < 2; $count++) {
	system("latex", $file);
}


my $sub = ".tex";

my $tosub = ".dvi";
my $string = $file;
$string =~ s/$sub/$tosub/;
system("dvipdf", $string);

my @torm = (".aux", ".toc", ".dvi", ".nav", ".log", ".snm", ".out");

foreach my $element (@torm) 
{
    $string = $file;
    $string =~ s/$sub/$element/;
    if (-e $string) {
	system("rm", "-f", $string);
	print "File $string erased\n"; 
    }
}



